Efficient Automatic Machine Learning via Design Graphs

Despite the success of automated machine learning (AutoML), which aims to find the best design, including the architecture of deep networks and hyper-parameters, conventional AutoML methods are computationally expensive and hardly provide insights into the relations of different model design choices. To tackle the challenges, we propose FALCON, an efficient sample-based method to search for the optimal model design. Our key insight is to model the design space of possible model designs as a design graph, where the nodes represent design choices, and the edges denote design similarities. FALCON features 1) a task-agnostic module, which performs message passing on the design graph via a Graph Neural Network (GNN), and 2) a task-specific module, which conducts label propagation of the known model performance information on the design graph. Both modules are combined to predict the design performances in the design space, navigating the search direction. We conduct extensive experiments on 27 node and graph classification tasks from various application domains, and an image classification task on the CIFAR-10 dataset. We empirically show that FALCON can efficiently obtain the well-performing designs for each task using only 30 explored nodes. Specifically, FALCON has a comparable time cost with the one-shot approaches while achieving an average improvement of 3.3% compared with the best baselines.

==> chapters/tables/image_clas_main.tex <==

\begin{table}[t]
    \centering
    \begin{tabular}{lcc}
    \toprule
    Method& Search Cost (GPU days) &Error\\
    \midrule 
    Random\\
    %&0.26&9.44 \\
    BO && \\
    SA && \\
    \midrule
    ENAS-micro& \\
    DARTS-micro& \\
    DARTS-micro-gumbel& \\
    \midrule 
    \ours\\
    %&0.31&7.13\\
    \bottomrule 
    \end{tabular}
    \vspace{5pt}
    \caption{Search results on CIFAR-10 dataset.}
\end{table}



==> chapters/tables/transfer.tex <==

\begin{table}[t]
    \centering
    \begin{tabular}{lcccc}
    \toprule
    &NCI-H23 & SW-620 & P388\\
    \midrule 
    LazyAverage
    &55.32%\std{4.37}
    &59.13%\std{3.02}
    &57.83%\std{6.95}
    \\
    LazyMax
    & 64.39
    & 65.77
    &70.92\\
    \midrule 
    \ours
    &66.62%\std{3.25}
    &66.58%\std{2.07}
    &77.01%\std{1.42}
    \\
    \ours-FineTuned
    & 70.75%\std{1.93}
    &68.30%\std{0.95}
    &78.40%\std{1.28}
    \\
    \midrule 
    Bruteforce
    & 72.67&69.26&78.75\\
    \bottomrule 
    \end{tabular}
    \vspace{5pt}
    \caption{Transferability Results. LazyAverage (LazyMax) denotes the average (maximum) task performance of directly applying the best design of each training task on the certrain task. Bruteforce denotes the best task performance using exhaustion search. Specifically, we fully trained at least 10\% and 1\% designsfor small and large design spaces in this paper.}
\end{table}





==> figures/backup.tex <==

% \begin{algorithm}[H]
%     \caption{MetaNAS: Sequential Semi-Supervised Learning for Automated Graph Learning.}
%     \label{alg:dir2}
%     \begin{algorithmic}[1]
%     \REQUIRE Design space $\mathcal{S}$; Selection budget $K$; Warm-up epoch $m$; \\Learning rate $\lambda$; Inner loop number $\ell$; Message passing coverage $M$.
%     \STATE $(\mathcal{N}=\{s_i\in \mathbb{R}^D\mid i=1,\ldots, n\}, \mathcal{E}\in \mathbb{R}^{D\times D}) \leftarrow$ Encoder$(\mathcal{S})$
%     \STATE $\Phi\leftarrow \emptyset$, $\mathcal{F} = \mathcal{N}$ 
%     \STATE $\mathcal{G}\leftarrow\emptyset$, $h_{\theta}\leftarrow$ CreateMetaGNN$(D, M)$
%     \STATE $s_t\leftarrow$ RandomSample$(\mathcal{N})$
%     \WHILE{$|\Phi|<K$}
%     \STATE $v_t \leftarrow$ the validation performance of $s_t$ after training $m$ epoch
%     \STATE  $\Phi\leftarrow \Phi\cup \{s_t\}$, $\mathcal{F} \leftarrow$ $M$-hop-Neighbors$(\Phi) $
%     \STATE $\mathcal{G}\leftarrow (\Phi\cup \mathcal{F}, \{\mathcal{E}_{i, j}\mid \{s_i, s_j\} \in \Phi\cup \mathcal{F}\})$ 
%     \STATE $\mathcal{P}\leftarrow h_{\theta}(\mathcal{G})$
%     \FOR{$k = 1,\ldots, \ell$}{}
%     \STATE $\theta\leftarrow \theta - \lambda\partial_{\theta} \sum_{s_i\in \Phi}\mathcal{L}(\mathcal{P}[s_i], v_i)$  \textcolor{mygreen}{\# Optimizing parameters of meta-model}
%     \ENDFOR
%     \STATE $s_t\leftarrow$ Sample$(\mathcal{F}, h_{\theta}(\mathcal{G})[\mathcal{F}])$ \textcolor{mygreen}{\# Infer structure performance distribution}
%     \ENDWHILE
%     \STATE Fully train the top max($\lceil 0.1*K\rceil$, 5) models in $\Phi$ with the highest validation performance.
%     \RETURN the best fully trained model.
%     \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
%      \caption{MetaNAS: Sequential Semi-Supervised Learning for Automated Graph Learning.}
%     \label{alg:dir2}
%     \begin{algorithmic}[1]
%     \REQUIRE Design space $\mathcal{S}$; Selection budget $K$; Warm-up epoch $m$;\\ Learning rate $\lambda$; Number of message passing layers $M$; Maximum connected component $C$.
%     \STATE $(\mathcal{N}=\{s_i\}_{i=1}^{N}, \mathcal{A}\in \mathbb{R}^{N\times N}) \leftarrow$ \textsc{Encoder}$(\mathcal{S})$
%     \STATE $\Phi=\{s_i\}_{i=1}^{C}\leftarrow$ \textsc{SampleUnconnected}$(\mathcal{N}, C)$ 
%     \STATE $\mathcal{F} \leftarrow$ \textsc{M-hop-Neighbors}$(\Phi)$
%      \STATE $\mathcal{G}\leftarrow (\Phi\cup \mathcal{F}, \mathcal{A}_{\Phi\cup \mathcal{F}})$ 
%      \STATE $h_{\theta}\leftarrow$ \textsc{CreateMetaGNN}$(M)$
%     \WHILE{$|\Phi|<K$}
%      \STATE $\mathcal{P}\leftarrow h_{\theta}(\mathcal{G})$ \textcolor{mygreen}{\# Infer structure performance distribution}
%      \STATE $s_t\leftarrow$ Sample$(\mathcal{F}, \mathcal{P}[\mathcal{F}])$ 
%     \STATE $v_t \leftarrow$ Validation performance after training $s_t$ from $m$ epoch
%      \STATE $\Phi\leftarrow \Phi\cup \{s_t\}$, $\mathcal{F} \leftarrow$ \textsc{M-hop-Neighbors}$(\Phi) $
%      \STATE $\mathcal{G}\leftarrow (\Phi\cup \mathcal{F}, \mathcal{A}_{\Phi\cup \mathcal{F}})$ 
%      \WHILE{not converge}
%      \STATE $\theta\leftarrow \theta - \lambda\partial_{\theta} \sum_{s_i\in \Phi}\mathcal{L}(h_{\theta}(\mathcal{G})[s_i], v_i)$ \textcolor{mygreen}{\# Optimizing parameters of meta-model}
%   \ENDWHILE
%   \ENDWHILE
%   \STATE Fully train the top max($\lceil 0.1*K\rceil$, 5) models in $\Phi$ with the highest validation performance.
%   \RETURN The best fully trained model.
%   \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
%     \caption{MetaNAS v2: Sequential Semi-supervised node repression with probabilistic sampling. Differences are highlighted.}
%     \label{alg:dir2}
%     \begin{algorithmic}[1]
%     \REQUIRE Candidate architecture $\mathcal{S}=\{s_1,\ldots, s_n\}$; Selection budget $K$; Warm-up epoch $m$; \\Learning rate $\lambda$; Inner loop number $\ell$.
%     \STATE $\Phi\leftarrow \emptyset$, \textcolor{teal}{$\Psi \leftarrow \{s_i:p_i=1/n|i=1,\ldots,n\}$}
%     \STATE $\mathcal{G}\leftarrow$ CreateMetaGraph$(\mathcal{S})$
%     \STATE $h_{\theta}\leftarrow$ CreateMetaGNN$(\mathcal{G})$
%     \WHILE{$|\Phi|<K$}
%     \STATE  \textcolor{teal}{Sample $s_t$ from $\Psi\sim \text{ Norm}(\mathcal{P}+\epsilon)$ }
%     \STATE Train $s_t$ for $m$ epoch
%     \STATE $v_t \leftarrow$ the estimated performance of $s_t$
%     \STATE  $\Phi\leftarrow \Phi\cup \{s_t: v_t\}, \Psi \leftarrow \Psi- \{s_t\}$
%     \FOR{$i = 1,\ldots, \ell$}{}
%     \STATE $\theta\leftarrow \theta - \lambda\partial_{\theta} \sum_{(s_i:v_i)\in \Phi}\mathcal{L}(h(s_i), v_i)$  
%     \ENDFOR
%     \STATE \textcolor{teal}{Update probability distribution: $\mathcal{P} \leftarrow \text{ Norm}(h(s_j)|j=1,\ldots,|\Psi|)$}
%     \ENDWHILE
%     \STATE Fully train the top $\lceil 0.1*K\rceil$ models in $\Phi$ with the highest validation performance.
%     \RETURN the best fully trained model.
%     \end{algorithmic}
% \end{algorithm}
